"I can assure you [$\ldots$] that it's going to be all right" -- A definition, case for, and survey of algorithmic assurances in human-autonomy trust relationships

As technology become more advanced, those who design, use and are otherwise affected by it want to know that it will perform correctly, and understand why it does what it does, and how to use it appropriately. In essence they want to be able to trust the systems that are being designed. In this survey we present assurances that are the method by which users can understand how to trust this technology. Trust between humans and autonomy is reviewed, and the implications for the design of assurances are highlighted. A survey of research that has been performed with respect to assurances is presented, and several key ideas are extracted in order to refine the definition of assurances. Several directions for future research are identified and discussed.

==> ass_cc.tex <==
\subsubsection{Component and Composite Assurances}
Assurances can be either component or composite. This was seen a little through the survey. The definitions are as follows:

\begin{description}
    \item [Component Assurance:] An assurance that originates from a single AIA capability source, and targets a single trust dimension target.
    \item [Composite Assurance:] The combination of more than one component assurance into a single assurance. 
\end{description}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/Assurance_component_composite.pdf}
    \caption{Figure illustrating the difference between component and composite assurances. The existence of multiple assurances does not imply a composite assurances, rather the combination of multiple component assurances into a single assurance constitutes a composite assurance.}
    \label{fig:assurance_mapping}
\end{figure}

Figure \ref{fig:assurance_mapping} illustrates the concepts of component and composite assurances.

\paragraph{Component Assurances:} Component assurances are perhaps the most well researched in the existing literature. This is likely because several verified component assurances are the predecessors to composite ones. A component assurance might include displaying the confidence of a classification prediction, or visualizing a model as discussed in section \ref{sec:q2}.

\paragraph{Composite Assurances:} Composite assurances are assurances that are built of several components. A notable example is the work by \citet{Aitken2016-cv} who propose a measurement called `self-confidence', applicable to Partially Observable Markov Decision Processes (POMDPs). This metric combines five component assurances into a single composite assurance that is meant to distill the information into a value that a novice operator could understand easily. This paper was discussed in more detail in \ref{sec:q2}. 


==> ass_ei.tex <==
\subsubsection{Explicit and Implicit Assurances}
As has already been presented, assurances can be either be \emph{explicit} or \emph{implicit}. This is something that \cite{Sheridan1984-kx} briefly alluded to in their discussion of the nature of how humans behave when working with automated systems. They suggested that the operator's perception of the automated system can be effected by `performance' and its `reports on its own performance'. This is an unnamed trend in the existing literature as well, as has been highlighted by the survey sections of this paper. Here the terms are more formally defined as (with some illustrative examples),

\begin{description}
    \item [Explicit Assurances:] Assurances that are purposefully given to affect the trust of a user.
    \begin{itemize}
        \item Legible motion \cite{Dragan2013-wd}, which is motion calculated with the intent of being more understandable by a human
        \item Self-confidence \cite{Aitken2016-fb}, a set of designed metrics meant to affect the user's trust
    \end{itemize}
    \item [Implicit Assurances:] All other assurances that aren't explicit.
    \begin{itemize}
        \item Reliability in completing a task. Generally, the object of success is not to affect the user's trust (although this is a nice side-effect).
        \item The way an autonomous vehicle appears. For example something that looks neat will have a different effect on trust, than an AIA with wires dragging on the ground. 
    \end{itemize}
\end{description}

While anything that affect the user's trust is seen as an assurances from their perspective, it is important for designers of AIAs to be aware of both kinds of assurances. Anything that is consciously designed with the goal of affecting trust is automatically an explicit assurance, from the perspective of the AIA. Another way of stating the idea is that trust relationships between humans and AIAs will form, but all assurances will be implicit if designers do not consciously consider the trust relationship. 
%
% Implicit assurances were the first that were formally researched in literature regarding human-AIA trust relationships. The research suggests that they are effective, and thus should be considered, however the real aim in designing for human-AIA trust relationships is to move toward the design of explicit assurances. Explicit does not mean that the user will always be aware of the communication (like in \cite{Dragan2013-wd}), but that there is a specifically designed method that has been shown to affect trust.


==> ass_st.tex <==
\subsubsection{Source-Target Classification}
    This is not a topic that was specifically reviewed in the survey (in fact it could have been another dimension along which to organize the survey), but we propose that it is convenient to refer to assurances by way of their source and target. More specifically their source AIA behavior (see Figure \ref{fig:AIcapabilities}) and their user trust target component (see figure \ref{fig:Assurance_classes}). Intuitively, there may be a set of different algorithms that are useful for making assurances that convey information about planning to the competence dimension of the user's trust. It is easier to refer to these assurances in terms of their source and target. So, for this example that class of algorithms would be the `planning-competence' class.

    The source AIA capability for an assurance might be most easily thought of by the algorithm it has to operate on. If the assurance operates on, or comes from, a planning algorithm then it would be considered a `planning' source. If the algorithm operated on data for learning patterns, the it would be considered a `learning' source.

    The trust dimensions shown in Figure \ref{fig:Assurance_classes} are the possible targets for assurances. The categories mirror those of the trust model proposed by \citet{McKnight2001-fa}, but with the emphasis on what an AIA has the ability to most readily influence (and consequently where most research is found). The boxes with the beveled corner identify and define the different classes of assurances. All classes are included here for completeness and generality, although, while it is hypothetically possible for an AIA to influence a persons general `Trusting stance' given enough time\footnote{One might imagine an AIA that specifically speaks to the human about the benefits or drawbacks about trusting even though there might not be evidence to do so, similar to the role a counselor might play}, the gray boxes were not considered in this survey, as practically no direct research exists in the realm of human-AIA relationships. However, as AIAs move further into quadrant IV. they will likely begin to have the ability to influence the dimensions that are greyed out.
    
    Not only is the source-target notation useful shorthand for communicating about the purpose of the assurance, but it is useful in classifying the range of assurance algorithms that exist. There may also be a class of algorithms that span multiple source-target capabilities. For example there may be a kind of algorithm that can give a `learning-competence' assurance, as well as a `planning-competence' assurance. This is especially true since many of the AIA capabilities can overlap. Also, the effects of assurances cannot be guaranteed to affect only one trust dimension (see section \ref{sec:imprecise}).

    In retrospect the reader may be able to identify work like \citet{Dragan2013-wd} as a `motion-predictability' assurance, or \cite{Wang2016-id} considered `perception-competence', and `planning-predictability' assurances (among others). \citet{Aitken2016-fb} considered a large set of assurances that span several source capabilities, and target trust dimensions.


==> ass_tt.tex <==
\subsubsection{Tutoring vs Telling} \label{sec:teach_tell}
    This is also a point rarely seen in the literature surveyed, but critical in the context of different users and long-term human-AIA interaction. We suggest that assurances can also be classified by whether they consider tutoring (or leading) the user to help them understand, or whether they just produce a static and unchanging value regardless of the user, their experience, or their expertise. This is a point mentioned (in terms of explainability) by \citet{Lacave2002-cu}, and \citet{Lacher2014-yc}.

    A tutoring assurance would be a planned, dynamic, sequence of assurances that would change in time to adapt to the user's needs (as discussed in section \ref{sec:consider_human}. This might include modification of assurances to help a user avoid boredom, or to use the system differently in varying circumstances. For example the first time an autonomous vehicle encounters snow with a certain user, it might take time to give special assurances. Or a user that is so used to an AIA that its TRBs begin to drift to disuse, and the AIA gives a special assurance to correct that.

    It isn't surprising that, to our knowledge, no research has been done with respect to tutoring a user in a trust relationship. This is a complex problem to address that would involve understanding how different users learn, and what an appropriate strategy would be to teach them to have appropriate TRBs. However, a rich resource (not investigated in this paper) would be the work on tutoring systems. There is definitely an open area for research that investigates the advantages of tutoring assurances versus those of telling assurances, and how easy they are to implement in contrast to the added time and effort needed to design tutoring assurances.

